2FA Sketch: Two-Factor Armor Sketch for Accurate and Efficient Heavy Hitter Detection in Data Streams

Detecting heavy hitters, which are flows exceeding a specified threshold, is crucial for network measurement, but it faces challenges due to increasing throughput and memory constraints. Existing sketch-based solutions, particularly those using Comparative Counter Voting, have limitations in efficiently identifying heavy hitters. This paper introduces the Two-Factor Armor (2FA) Sketch, a novel data structure designed to enhance heavy hitter detection in data streams. 2FA Sketch implements dual-layer protection through an improved $\mathtt{Arbitration}$ strategy for in-bucket competition and a cross-bucket conflict $\mathtt{Avoidance}$ hashing scheme. By theoretically deriving an optimal $\lambda$ parameter and redesigning $vote^+_{new}$ as a conflict indicator, it optimizes the Comparative Counter Voting strategy. Experimental results show that 2FA Sketch outperforms the standard Elastic Sketch, reducing error rates by 2.5 to 19.7 times and increasing processing speed by 1.03 times.

==> InputFiles/author_format.tex <==
\author{Tong Yang, Gaogang xie, Yanbiao Li, Qiaobin Fu, Alex X. Liu, Qi Li, Laurent Mathy}

\numberofauthors{6}
\author{
\alignauthor
Tong Yang,Gaogang Xie*\\
       %\affaddr{Institute of Computing Technology, Chinese Academy of Sciences (CAS), China.}\\
       \affaddr{ICT, CAS, China.}\\
       \email{yangtongemail@gmail.com, *xie@ict.ac.cn}
\alignauthor
YanBiao Li\\
       %\affaddr{College of Computer Science and Electronic Engineering, Hunan University, China}\\
       \affaddr{Hunan University, China}\\
       \email{lybmath\_cs@hnu.edu.cn}
\alignauthor
Qiaobin Fu\\
       \affaddr{ICT, CAS, China}\\
       \email{fuqiaobin@ict.ac.cn}
\and
\alignauthor Alex X. Liu\\
       \affaddr{Department of Computer Science and Engineering, Michigan State University}\\
       \email{alexliu@cse.msu.edu}
\alignauthor Qi Li\\
       \affaddr{ICT, CAS, China}\\
       \email{liqi19872006@gmail.com}
\alignauthor Laurent Mathy\\
       \affaddr{University of Liege, Belgium}\\
       \email{laurent.mathy@ulg.ac.be}
}


\author{\IEEEauthorblockN{Tong Yang\IEEEauthorrefmark{1},
Xiaoming Li\IEEEauthorrefmark{1},
Alex X. Liu\IEEEauthorrefmark{2},
Qiaobin Fu\IEEEauthorrefmark{3},
Gaogang Xie\IEEEauthorrefmark{4}}
\IEEEauthorblockA{\IEEEauthorrefmark{1}Computer Science Department, Peking University, Beijing, China}
\IEEEauthorblockA{\IEEEauthorrefmark{2}Department of Computer Science and Engineering, Michigan State University}
\IEEEauthorblockA{\IEEEauthorrefmark{3}Computer Science Department, Boston University, USA}
\IEEEauthorblockA{\IEEEauthorrefmark{4}ICT, CAS, China}
}
